Fantastic flat bands and where to find them: The CoSn-type compounds

Quantum interference on the kagome lattice generates electronic bands with narrow bandwidth, called flat bands. Crystal structures incorporating this lattice can host strong electron correlations with non-standard ingredients, but only if these bands lie at the Fermi level. In the six compounds with the CoSn structure type (FeGe, FeSn, CoSn, NiIn, RhPb, and PtTl) the transition metals form a kagome lattice. The two iron variants are robust antiferromagnets so we focus on the latter four and investigate their thermodynamic and transport properties. We consider these results and calculated band structures to locate and characterize the flat bands in these materials. We propose that CoSn and RhPb deserve the community's attention for exploring flat band physics.

==> CoSn-Type_Kagome_Metals_10_sub.bbl.tex <==
%apsrev4-2.bst 2019-01-14 (MD) hand-edited version of apsrev4-1.bst
%Control: key (0)
%Control: author (8) initials jnrlst
%Control: editor formatted (1) identically to author
%Control: production of article title (0) allowed
%Control: page (0) single
%Control: year (1) truncated
%Control: production of eprint (0) enabled
\begin{thebibliography}{60}%
\makeatletter
\providecommand \@ifxundefined [1]{%
 \@ifx{#1\undefined}
}%
\providecommand \@ifnum [1]{%
 \ifnum #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \@ifx [1]{%
 \ifx #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \natexlab [1]{#1}%
\providecommand \enquote  [1]{``#1''}%
\providecommand \bibnamefont  [1]{#1}%
\providecommand \bibfnamefont [1]{#1}%
\providecommand \citenamefont [1]{#1}%
\providecommand \href@noop [0]{\@secondoftwo}%
\providecommand \href [0]{\begingroup \@sanitize@url \@href}%
\providecommand \@href[1]{\@@startlink{#1}\@@href}%
\providecommand \@@href[1]{\endgroup#1\@@endlink}%
\providecommand \@sanitize@url [0]{\catcode `\\12\catcode `\$12\catcode
  `\&12\catcode `\#12\catcode `\^12\catcode `\_12\catcode `\%12\relax}%
\providecommand \@@startlink[1]{}%
\providecommand \@@endlink[0]{}%
\providecommand \url  [0]{\begingroup\@sanitize@url \@url }%
\providecommand \@url [1]{\endgroup\@href {#1}{\urlprefix }}%
\providecommand \urlprefix  [0]{URL }%
\providecommand \Eprint [0]{\href }%
\providecommand \doibase [0]{https://doi.org/}%
\providecommand \selectlanguage [0]{\@gobble}%
\providecommand \bibinfo  [0]{\@secondoftwo}%
\providecommand \bibfield  [0]{\@secondoftwo}%
\providecommand \translation [1]{[#1]}%
\providecommand \BibitemOpen [0]{}%
\providecommand \bibitemStop [0]{}%
\providecommand \bibitemNoStop [0]{.\EOS\space}%
\providecommand \EOS [0]{\spacefactor3000\relax}%
\providecommand \BibitemShut  [1]{\csname bibitem#1\endcsname}%
\let\auto@bib@innerbib\@empty
%</preamble>
\bibitem [{\citenamefont {Kittel}(2004)}]{Kittel2004_SolidStatePhysics}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.}~\bibnamefont
  {Kittel}},\ }\href
  {https://www.ebook.de/de/product/4290142/charles_kittel_introduction_to_solid_state_physics.html}
  {\emph {\bibinfo {title} {Introduction to solid state physics}}},\ \bibinfo
  {edition} {eighth}\ ed.\ (\bibinfo  {publisher} {John Wiley \& Sons Inc},\
  \bibinfo {year} {2004})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Grosso}\ and\ \citenamefont
  {Parravicini}(2014)}]{Grosso2014_SolidStatePhysics}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Grosso}}\ and\ \bibinfo {author} {\bibfnamefont {G.~P.}\ \bibnamefont
  {Parravicini}},\ }\href
  {https://www.ebook.de/de/product/20340579/giuseppe_grosso_solid_state_physics.html}
  {\emph {\bibinfo {title} {Solid state physics}}},\ \bibinfo {edition} {2nd}\
  ed.\ (\bibinfo  {publisher} {Elsevier LTD, Oxford, UK},\ \bibinfo {year}
  {2014})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Leykam}\ \emph {et~al.}(2018)\citenamefont {Leykam},
  \citenamefont {Andreanov},\ and\ \citenamefont
  {Flach}}]{Leykam2018_ArtificialFlatBandSystems}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Leykam}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Andreanov}},\
  and\ \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Flach}},\ }\bibfield
   {title} {\bibinfo {title} {Artificial flat band systems: from lattice models
  to experiments},\ }\href {https://doi.org/10.1080/23746149.2018.1473052}
  {\bibfield  {journal} {\bibinfo  {journal} {Advances in Physics: X}\ }\textbf
  {\bibinfo {volume} {3}},\ \bibinfo {pages} {1473052} (\bibinfo {year}
  {2018})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont
  {Sutherland}(1986)}]{Sutherland1986_LocalizationOfElectronicWaveFunctionsDueToLocalTopology}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Sutherland}},\ }\bibfield  {title} {\bibinfo {title} {Localization of
  electronic wave functions due to local topology},\ }\href
  {https://doi.org/10.1103/physrevb.34.5208} {\bibfield  {journal} {\bibinfo
  {journal} {Physical Review B}\ }\textbf {\bibinfo {volume} {34}},\ \bibinfo
  {pages} {5208} (\bibinfo {year} {1986})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Cao}\ \emph {et~al.}(2018{\natexlab{a}})\citenamefont
  {Cao}, \citenamefont {Fatemi}, \citenamefont {Demir}, \citenamefont {Fang},
  \citenamefont {Tomarken}, \citenamefont {Luo}, \citenamefont
  {Sanchez-Yamagishi}, \citenamefont {Watanabe}, \citenamefont {Taniguchi},
  \citenamefont {Kaxiras}, \citenamefont {Ashoori},\ and\ \citenamefont
  {Jarillo-Herrero}}]{Cao2018_CorrelatedInsulatorMagicAngleTwistedBilayerGraphene}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont
  {Cao}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Fatemi}},
  \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Demir}}, \bibinfo
  {author} {\bibfnamefont {S.}~\bibnamefont {Fang}}, \bibinfo {author}
  {\bibfnamefont {S.~L.}\ \bibnamefont {Tomarken}}, \bibinfo {author}
  {\bibfnamefont {J.~Y.}\ \bibnamefont {Luo}}, \bibinfo {author} {\bibfnamefont
  {J.~D.}\ \bibnamefont {Sanchez-Yamagishi}}, \bibinfo {author} {\bibfnamefont
  {K.}~\bibnamefont {Watanabe}}, \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {Taniguchi}}, \bibinfo {author} {\bibfnamefont
  {E.}~\bibnamefont {Kaxiras}}, \bibinfo {author} {\bibfnamefont {R.~C.}\
  \bibnamefont {Ashoori}},\ and\ \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {Jarillo-Herrero}},\ }\bibfield  {title} {\bibinfo {title}
  {Correlated insulator behaviour at half-filling in magic-angle graphene
  superlattices},\ }\href {https://doi.org/10.1038/nature26154} {\bibfield
  {journal} {\bibinfo  {journal} {Nature}\ }\textbf {\bibinfo {volume} {556}},\
  \bibinfo {pages} {80} (\bibinfo {year} {2018}{\natexlab{a}})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Cao}\ \emph {et~al.}(2018{\natexlab{b}})\citenamefont
  {Cao}, \citenamefont {Fatemi}, \citenamefont {Fang}, \citenamefont
  {Watanabe}, \citenamefont {Taniguchi}, \citenamefont {Kaxiras},\ and\
  \citenamefont
  {Jarillo-Herrero}}]{Cao2018_UnconventionalSuperconductivityMagicAngleTwistedBilayerGraphene}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont
  {Cao}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Fatemi}},
  \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Fang}}, \bibinfo {author}
  {\bibfnamefont {K.}~\bibnamefont {Watanabe}}, \bibinfo {author}
  {\bibfnamefont {T.}~\bibnamefont {Taniguchi}}, \bibinfo {author}
  {\bibfnamefont {E.}~\bibnamefont {Kaxiras}},\ and\ \bibinfo {author}
  {\bibfnamefont {P.}~\bibnamefont {Jarillo-Herrero}},\ }\bibfield  {title}
  {\bibinfo {title} {Unconventional superconductivity in magic-angle graphene
  superlattices},\ }\href {https://doi.org/10.1038/nature26160} {\bibfield
  {journal} {\bibinfo  {journal} {Nature}\ }\textbf {\bibinfo {volume} {556}},\
  \bibinfo {pages} {43} (\bibinfo {year} {2018}{\natexlab{b}})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Sun}\ \emph {et~al.}(2011)\citenamefont {Sun},
  \citenamefont {Gu}, \citenamefont {Katsura},\ and\ \citenamefont
  {Sarma}}]{Sun2011_NearlyFlatbandsWithNontrivialTopology}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Sun}}, \bibinfo {author} {\bibfnamefont {Z.}~\bibnamefont {Gu}}, \bibinfo
  {author} {\bibfnamefont {H.}~\bibnamefont {Katsura}},\ and\ \bibinfo {author}
  {\bibfnamefont {S.~D.}\ \bibnamefont {Sarma}},\ }\bibfield  {title} {\bibinfo
  {title} {Nearly flatbands with nontrivial topology},\ }\bibfield  {journal}
  {\bibinfo  {journal} {Physical Review Letters}\ }\textbf {\bibinfo {volume}
  {106}},\ \href {https://doi.org/10.1103/physrevlett.106.236803}
  {10.1103/physrevlett.106.236803} (\bibinfo {year} {2011})\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Momma}\ and\ \citenamefont
  {Izumi}(2011)}]{Momma2011_Vesta3}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Momma}}\ and\ \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Izumi}},\
  }\bibfield  {title} {\bibinfo {title} {{VESTA}3 for three-dimensional
  visualization of crystal, volumetric and morphology data},\ }\href
  {https://doi.org/10.1107/s0021889811038970} {\bibfield  {journal} {\bibinfo
  {journal} {Journal of Applied Crystallography}\ }\textbf {\bibinfo {volume}
  {44}},\ \bibinfo {pages} {1272} (\bibinfo {year} {2011})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Beugeling}\ \emph {et~al.}(2012)\citenamefont
  {Beugeling}, \citenamefont {Everts},\ and\ \citenamefont
  {Smith}}]{Beugeling2012_TopologicalNNNHoppingIn2DLattice}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {W.}~\bibnamefont
  {Beugeling}}, \bibinfo {author} {\bibfnamefont {J.~C.}\ \bibnamefont
  {Everts}},\ and\ \bibinfo {author} {\bibfnamefont {C.~M.}\ \bibnamefont
  {Smith}},\ }\bibfield  {title} {\bibinfo {title} {Topological phase
  transitions driven by next-nearest-neighbor hopping in two-dimensional
  lattices},\ }\bibfield  {journal} {\bibinfo  {journal} {Physical Review B}\
  }\textbf {\bibinfo {volume} {86}},\ \href
  {https://doi.org/10.1103/physrevb.86.195129} {10.1103/physrevb.86.195129}
  (\bibinfo {year} {2012})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kang}\ \emph {et~al.}(2019)\citenamefont {Kang},
  \citenamefont {Ye}, \citenamefont {Fang}, \citenamefont {You}, \citenamefont
  {Levitan}, \citenamefont {Han}, \citenamefont {Facio}, \citenamefont
  {Jozwiak}, \citenamefont {Bostwick}, \citenamefont {Rotenberg}, \citenamefont
  {Chan}, \citenamefont {McDonald}, \citenamefont {Graf}, \citenamefont
  {Kaznatcheev}, \citenamefont {Vescovo}, \citenamefont {Bell}, \citenamefont
  {Kaxiras}, \citenamefont {van~den Brink}, \citenamefont {Richter},
  \citenamefont {Ghimire}, \citenamefont {Checkelsky},\ and\ \citenamefont
  {Comin}}]{Kang2019_DiracAndFlatBandsFeSn}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Kang}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Ye}}, \bibinfo
  {author} {\bibfnamefont {S.}~\bibnamefont {Fang}}, \bibinfo {author}
  {\bibfnamefont {J.-S.}\ \bibnamefont {You}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Levitan}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Han}}, \bibinfo {author} {\bibfnamefont {J.~I.}\
  \bibnamefont {Facio}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont
  {Jozwiak}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Bostwick}},
  \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Rotenberg}}, \bibinfo
  {author} {\bibfnamefont {M.~K.}\ \bibnamefont {Chan}}, \bibinfo {author}
  {\bibfnamefont {R.~D.}\ \bibnamefont {McDonald}}, \bibinfo {author}
  {\bibfnamefont {D.}~\bibnamefont {Graf}}, \bibinfo {author} {\bibfnamefont
  {K.}~\bibnamefont {Kaznatcheev}}, \bibinfo {author} {\bibfnamefont
  {E.}~\bibnamefont {Vescovo}}, \bibinfo {author} {\bibfnamefont {D.~C.}\
  \bibnamefont {Bell}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Kaxiras}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {van~den
  Brink}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Richter}},
  \bibinfo {author} {\bibfnamefont {M.~P.}\ \bibnamefont {Ghimire}}, \bibinfo
  {author} {\bibfnamefont {J.~G.}\ \bibnamefont {Checkelsky}},\ and\ \bibinfo
  {author} {\bibfnamefont {R.}~\bibnamefont {Comin}},\ }\bibfield  {title}
  {\bibinfo {title} {Dirac fermions and flat bands in the ideal kagome metal
  {F}e{S}n},\ }\href {https://doi.org/10.1038/s41563-019-0531-0} {\bibfield
  {journal} {\bibinfo  {journal} {Nature Materials}\ }\textbf {\bibinfo
  {volume} {19}},\ \bibinfo {pages} {163} (\bibinfo {year} {2019})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Kang}\ \emph {et~al.}(2020)\citenamefont {Kang},
  \citenamefont {Fang}, \citenamefont {Ye}, \citenamefont {Po}, \citenamefont
  {Denlinger}, \citenamefont {Jozwiak}, \citenamefont {Bostwick}, \citenamefont
  {Rotenberg}, \citenamefont {Kaxiras}, \citenamefont {Checkelsky},\ and\
  \citenamefont {Comin}}]{Kang2020_TopologicalFlatBandsCoSnARPES}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Kang}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Fang}}, \bibinfo
  {author} {\bibfnamefont {L.}~\bibnamefont {Ye}}, \bibinfo {author}
  {\bibfnamefont {H.~C.}\ \bibnamefont {Po}}, \bibinfo {author} {\bibfnamefont
  {J.}~\bibnamefont {Denlinger}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Jozwiak}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Bostwick}}, \bibinfo {author} {\bibfnamefont
  {E.}~\bibnamefont {Rotenberg}}, \bibinfo {author} {\bibfnamefont
  {E.}~\bibnamefont {Kaxiras}}, \bibinfo {author} {\bibfnamefont {J.~G.}\
  \bibnamefont {Checkelsky}},\ and\ \bibinfo {author} {\bibfnamefont
  {R.}~\bibnamefont {Comin}},\ }\bibfield  {title} {\bibinfo {title}
  {Topological flat bands in frustrated kagome lattice {CoSn}},\ }\href@noop {}
  {\  (\bibinfo {year} {2020})},\ \Eprint {https://arxiv.org/abs/2002.01452v1}
  {2002.01452v1} \BibitemShut {NoStop}%
\bibitem [{\citenamefont {Liu}\ \emph {et~al.}()\citenamefont {Liu},
  \citenamefont {Li}, \citenamefont {Wang}, \citenamefont {Wang}, \citenamefont
  {Wen}, \citenamefont {Jiang}, \citenamefont {Lu}, \citenamefont {Yan},
  \citenamefont {Huang}, \citenamefont {Shen}, \citenamefont {Yin},
  \citenamefont {Wang}, \citenamefont {Yin}, \citenamefont {Lei},\ and\
  \citenamefont {Wang}}]{Liu2020_DiracFermionsFlatBandsCoSn_ARPES}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Z.}~\bibnamefont
  {Liu}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Li}}, \bibinfo
  {author} {\bibfnamefont {Q.}~\bibnamefont {Wang}}, \bibinfo {author}
  {\bibfnamefont {G.}~\bibnamefont {Wang}}, \bibinfo {author} {\bibfnamefont
  {C.~H.~P.}\ \bibnamefont {Wen}}, \bibinfo {author} {\bibfnamefont
  {K.}~\bibnamefont {Jiang}}, \bibinfo {author} {\bibfnamefont
  {X.}~\bibnamefont {Lu}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Yan}}, \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Huang}}, \bibinfo
  {author} {\bibfnamefont {D.}~\bibnamefont {Shen}}, \bibinfo {author}
  {\bibfnamefont {J.}~\bibnamefont {Yin}}, \bibinfo {author} {\bibfnamefont
  {Z.}~\bibnamefont {Wang}}, \bibinfo {author} {\bibfnamefont {Z.}~\bibnamefont
  {Yin}}, \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Lei}},\ and\
  \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Wang}},\ }\bibfield
  {title} {\bibinfo {title} {Orbital-selective {D}irac fermions and extremely
  flat bands in the nonmagnetic kagome metal {CoSn}},\ }\href@noop {} {\
  }\Eprint {https://arxiv.org/abs/2001.11738v1} {2001.11738v1} \BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Villars}\ and\ \citenamefont
  {Cenzual}(2014)}]{Villars2012_PearsonCrystalDatabase}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Villars}}\ and\ \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Cenzual}},\ }\bibfield  {title} {\bibinfo {title} {Pearson’s crystal
  data-crystal structure database for inorganic compounds},\ }\href@noop {}
  {\bibfield  {journal} {\bibinfo  {journal} {ASM International, Materials
  Park, Ohio, USA}\ } (\bibinfo {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bergerhoff}\ and\ \citenamefont
  {Brown}(1987)}]{Bergerhoff1987_ICSD}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Bergerhoff}}\ and\ \bibinfo {author} {\bibfnamefont {I.~D.}\ \bibnamefont
  {Brown}},\ }\bibfield  {title} {\bibinfo {title} {Crystallographic
  databases},\ }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal}
  {International Union of Crystallography, Chester}\ }\textbf {\bibinfo
  {volume} {360}},\ \bibinfo {pages} {77} (\bibinfo {year} {1987})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont
  {Richardson}(1967)}]{Richardson1967_EquilibriumDiagram_FeGe_System}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Richardson}},\ }\bibfield  {title} {\bibinfo {title} {The partial
  equilibrium diagram of the {Fe}-{Ge} system in the range 40-72 at. {\%} {Ge},
  and the crystallisation of some iron germanides by chemical transport
  reactions},\ }\href {https://doi.org/10.3891/acta.chem.scand.21-2305}
  {\bibfield  {journal} {\bibinfo  {journal} {Acta Chemica Scandinavica}\
  }\textbf {\bibinfo {volume} {21}},\ \bibinfo {pages} {2305} (\bibinfo {year}
  {1967})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont
  {Nial}(1945)}]{Nial1945_XrayStudiesOfBinaryAlloysOfTin}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {O.}~\bibnamefont
  {Nial}},\ }\emph {\bibinfo {title} {X-ray studies on binary alloys of tin
  with transition metals}},\ \href {https://pubs.sub.su.se/1714.pdf} {Ph.D.
  thesis},\ \bibinfo  {school} {Stockholm College} (\bibinfo {year}
  {1945})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hellner}\ and\ \citenamefont
  {Laves}(1947)}]{Hellner1947_InGaCompoundsWithNiPdPtCuAgAu}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Hellner}}\ and\ \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Laves}},\ }\bibfield  {title} {\bibinfo {title} {Kristallchemie des {In} und
  {Ga} in legierungen mit einigen \"ubergangselementen ({Ni}, {Pd}, {Pt}, {Cu},
  {Ag} und {Au})},\ }\href {https://doi.org/10.1515/zna-1947-0310} {\bibfield
  {journal} {\bibinfo  {journal} {Zeitschrift für Naturforschung A}\ }\textbf
  {\bibinfo {volume} {2}},\ \bibinfo {pages} {177} (\bibinfo {year}
  {1947})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {El-Boragy}\ \emph {et~al.}(1972)\citenamefont
  {El-Boragy}, \citenamefont {Jain}, \citenamefont {Mayer},\ and\ \citenamefont
  {Schubert}}]{ElBoragy1972_Rh-Pb}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {El-Boragy}}, \bibinfo {author} {\bibfnamefont {K.~C.}\ \bibnamefont {Jain}},
  \bibinfo {author} {\bibfnamefont {H.~W.}\ \bibnamefont {Mayer}},\ and\
  \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Schubert}},\ }\bibfield
  {title} {\bibinfo {title} {Zur konstitution der mischung rhodium-blei},\
  }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Z Metallkd}\
  }\textbf {\bibinfo {volume} {63}},\ \bibinfo {pages} {751} (\bibinfo {year}
  {1972})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Zintl}\ and\ \citenamefont
  {Harder}(1935)}]{Zintl1935_StructPlatinumThallium}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Zintl}}\ and\ \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Harder}},\
  }\bibfield  {title} {\bibinfo {title} {Struktur der
  platin‐thallium‐legierungen},\ }\href@noop {} {\bibfield  {journal}
  {\bibinfo  {journal} {Zeitschrift f\"ur Elektrochemie und angewandte
  physikalische Chemie}\ }\textbf {\bibinfo {volume} {41}},\ \bibinfo {pages}
  {767} (\bibinfo {year} {1935})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Beckman}\ \emph {et~al.}(1972)\citenamefont
  {Beckman}, \citenamefont {Carrander}, \citenamefont {Lundgren},\ and\
  \citenamefont {Richardson}}]{Beckman1972_hexFeGe_MagSusceptAndOrdering}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {O.}~\bibnamefont
  {Beckman}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Carrander}},
  \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Lundgren}},\ and\
  \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Richardson}},\ }\bibfield
   {title} {\bibinfo {title} {Susceptibility measurements and magnetic ordering
  of hexagonal {FeGe}},\ }\href {https://doi.org/10.1088/0031-8949/6/2-3/009}
  {\bibfield  {journal} {\bibinfo  {journal} {Physica Scripta}\ }\textbf
  {\bibinfo {volume} {6}},\ \bibinfo {pages} {151} (\bibinfo {year}
  {1972})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Beckman}\ \emph {et~al.}(1973)\citenamefont
  {Beckman}, \citenamefont {Sundstr\"om}, \citenamefont {Carrander},\ and\
  \citenamefont {Lundgren}}]{Beckman1973_LocalVsItinerantInHexFeGe}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {O.}~\bibnamefont
  {Beckman}}, \bibinfo {author} {\bibfnamefont {L.~J.}\ \bibnamefont
  {Sundstr\"om}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Carrander}},\ and\ \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont
  {Lundgren}},\ }\bibfield  {title} {\bibinfo {title} {Localized versus
  itinerant electrons in hexagonal {FeGe}},\ }\href
  {https://doi.org/10.1016/0038-1098(73)90037-9} {\bibfield  {journal}
  {\bibinfo  {journal} {Solid State Communications}\ }\textbf {\bibinfo
  {volume} {12}},\ \bibinfo {pages} {1061} (\bibinfo {year}
  {1973})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bernhard}\ \emph {et~al.}(1984)\citenamefont
  {Bernhard}, \citenamefont {Lebech},\ and\ \citenamefont
  {Beckman}}]{Bernhard1984_LowTempAFM_FeGe}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Bernhard}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Lebech}},\
  and\ \bibinfo {author} {\bibfnamefont {O.}~\bibnamefont {Beckman}},\
  }\bibfield  {title} {\bibinfo {title} {Neutron diffraction studies of the
  low-temperature magnetic structure of hexagonal {FeGe}},\ }\href
  {https://doi.org/10.1088/0305-4608/14/10/017} {\bibfield  {journal} {\bibinfo
   {journal} {Journal of Physics F: Metal Physics}\ }\textbf {\bibinfo {volume}
  {14}},\ \bibinfo {pages} {2379} (\bibinfo {year} {1984})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Bernhard}\ \emph {et~al.}(1988)\citenamefont
  {Bernhard}, \citenamefont {Lebech},\ and\ \citenamefont
  {Beckman}}]{Bernhard1988_MagneticPhaseDiagramFeGe}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Bernhard}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Lebech}},\
  and\ \bibinfo {author} {\bibfnamefont {O.}~\bibnamefont {Beckman}},\
  }\bibfield  {title} {\bibinfo {title} {Magnetic phase diagram of hexagonal
  {FeGe} determined by neutron diffraction},\ }\href
  {https://doi.org/10.1088/0305-4608/18/3/023} {\bibfield  {journal} {\bibinfo
  {journal} {Journal of Physics F: Metal Physics}\ }\textbf {\bibinfo {volume}
  {18}},\ \bibinfo {pages} {539} (\bibinfo {year} {1988})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Forsyth}\ \emph {et~al.}(1978)\citenamefont
  {Forsyth}, \citenamefont {Wilkinson},\ and\ \citenamefont
  {Gardner}}]{Forsyth1978_LowTempAFM_hexFeGe}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~B.}\ \bibnamefont
  {Forsyth}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Wilkinson}},\
  and\ \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Gardner}},\
  }\bibfield  {title} {\bibinfo {title} {The low-temperature magnetic structure
  of hexagonal {FeGe}},\ }\href {https://doi.org/10.1088/0305-4608/8/10/019}
  {\bibfield  {journal} {\bibinfo  {journal} {Journal of Physics F: Metal
  Physics}\ }\textbf {\bibinfo {volume} {8}},\ \bibinfo {pages} {2195}
  (\bibinfo {year} {1978})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {H\"aggström}\ \emph {et~al.}(1975)\citenamefont
  {H\"aggström}, \citenamefont {Ericsson}, \citenamefont {W\"appling},\ and\
  \citenamefont {Karlsson}}]{Haeggstroem1975_Mossbauer_hexFeGe}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {L.}~\bibnamefont
  {H\"aggström}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Ericsson}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {W\"appling}},\ and\ \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Karlsson}},\ }\bibfield  {title} {\bibinfo {title} {M\"ossbauer study of
  hexagonal {FeGe}},\ }\href {https://doi.org/10.1088/0031-8949/11/1/009}
  {\bibfield  {journal} {\bibinfo  {journal} {Physica Scripta}\ }\textbf
  {\bibinfo {volume} {11}},\ \bibinfo {pages} {55} (\bibinfo {year}
  {1975})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Stenstr\"om}\ \emph {et~al.}(1972)\citenamefont
  {Stenstr\"om}, \citenamefont {Sundstr\"om},\ and\ \citenamefont
  {Sagredo}}]{Stenstroem1972_ResistivityHexFeGe}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Stenstr\"om}}, \bibinfo {author} {\bibfnamefont {L.~J.}\ \bibnamefont
  {Sundstr\"om}},\ and\ \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont
  {Sagredo}},\ }\bibfield  {title} {\bibinfo {title} {The electrical
  resistivity of hexagonal {FeGe} single crystals},\ }\href
  {https://doi.org/10.1088/0031-8949/6/4/007} {\bibfield  {journal} {\bibinfo
  {journal} {Physica Scripta}\ }\textbf {\bibinfo {volume} {6}},\ \bibinfo
  {pages} {209} (\bibinfo {year} {1972})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Yamamoto}(1966)}]{Yamamoto1966_MossbauerFe5Sn3+FeSn}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {H.}~\bibnamefont
  {Yamamoto}},\ }\bibfield  {title} {\bibinfo {title} {{M}\"ossbauer effect
  measurement of intermetallic compounds in iron-tin system : {F}e$_5${S}n$_3$
  and {FeSn}},\ }\href {https://doi.org/10.1143/jpsj.21.1058} {\bibfield
  {journal} {\bibinfo  {journal} {Journal of the Physical Society of Japan}\
  }\textbf {\bibinfo {volume} {21}},\ \bibinfo {pages} {1058} (\bibinfo {year}
  {1966})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Yamaguchi}\ and\ \citenamefont
  {Watanabe}(1967)}]{Yamaguchi1967_FeSnNeutronDiffraction}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Yamaguchi}}\ and\ \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont
  {Watanabe}},\ }\bibfield  {title} {\bibinfo {title} {Neutron diffraction
  study of {FeSn}},\ }\href {https://doi.org/10.1143/jpsj.22.1210} {\bibfield
  {journal} {\bibinfo  {journal} {Journal of the Physical Society of Japan}\
  }\textbf {\bibinfo {volume} {22}},\ \bibinfo {pages} {1210} (\bibinfo {year}
  {1967})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Sales}\ \emph {et~al.}(2019)\citenamefont {Sales},
  \citenamefont {Yan}, \citenamefont {Meier}, \citenamefont {Christianson},
  \citenamefont {Okamoto},\ and\ \citenamefont
  {McGuire}}]{Sales2019_2DMagnetismFeSn}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.~C.}\ \bibnamefont
  {Sales}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Yan}}, \bibinfo
  {author} {\bibfnamefont {W.~R.}\ \bibnamefont {Meier}}, \bibinfo {author}
  {\bibfnamefont {A.~D.}\ \bibnamefont {Christianson}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {Okamoto}},\ and\ \bibinfo {author}
  {\bibfnamefont {M.~A.}\ \bibnamefont {McGuire}},\ }\bibfield  {title}
  {\bibinfo {title} {Electronic, magnetic, and thermodynamic properties of the
  kagome layer compound {FeSn}},\ }\href
  {https://doi.org/10.1103/PhysRevMaterials.3.114203} {\bibfield  {journal}
  {\bibinfo  {journal} {Physical Review Materials}\ }\textbf {\bibinfo {volume}
  {3}},\ \bibinfo {pages} {114203} (\bibinfo {year} {2019})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Meier}\ \emph {et~al.}(2019)\citenamefont {Meier},
  \citenamefont {Yan}, \citenamefont {McGuire}, \citenamefont {Wang},
  \citenamefont {Christianson},\ and\ \citenamefont
  {Sales}}]{Meier2019_AFM_ReorientationCoDopedFeSn}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {W.~R.}\ \bibnamefont
  {Meier}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Yan}}, \bibinfo
  {author} {\bibfnamefont {M.~A.}\ \bibnamefont {McGuire}}, \bibinfo {author}
  {\bibfnamefont {X.}~\bibnamefont {Wang}}, \bibinfo {author} {\bibfnamefont
  {A.~D.}\ \bibnamefont {Christianson}},\ and\ \bibinfo {author} {\bibfnamefont
  {B.~C.}\ \bibnamefont {Sales}},\ }\bibfield  {title} {\bibinfo {title}
  {Reorientation of antiferromagnetism in cobalt doped {FeSn}},\ }\bibfield
  {journal} {\bibinfo  {journal} {Physical Review B}\ }\textbf {\bibinfo
  {volume} {100}},\ \href {https://doi.org/10.1103/physrevb.100.184421}
  {10.1103/physrevb.100.184421} (\bibinfo {year} {2019})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ligenza}(1972)}]{Ligenza1972_SnMossbauerFeSn}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Ligenza}},\ }\bibfield  {title} {\bibinfo {title} {A {M}\"ossbauer study of
  hyperfine parameters of {S}n119 in antiferromagnetic and paramagnetic states
  of {FeSn}},\ }\href {https://doi.org/10.1002/pssb.2220500144} {\bibfield
  {journal} {\bibinfo  {journal} {Physica Status Solidi (b)}\ }\textbf
  {\bibinfo {volume} {50}},\ \bibinfo {pages} {379} (\bibinfo {year}
  {1972})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ligenza}(1971)}]{Ligenza1971_SpinFlipFeSn}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Ligenza}},\ }\bibfield  {title} {\bibinfo {title} {A spin-flip effect in
  {FeSn}},\ }\href {https://doi.org/10.1002/pssb.2220450236} {\bibfield
  {journal} {\bibinfo  {journal} {Physica Status Solidi (b)}\ }\textbf
  {\bibinfo {volume} {45}},\ \bibinfo {pages} {721} (\bibinfo {year}
  {1971})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {H\"aggstr\"om}\ \emph {et~al.}(1975)\citenamefont
  {H\"aggstr\"om}, \citenamefont {Ericsson}, \citenamefont {W\'appling},\ and\
  \citenamefont {Chandra}}]{Haggstrom1975_MossbauerFeSn}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {L.}~\bibnamefont
  {H\"aggstr\"om}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Ericsson}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {W\'appling}},\ and\ \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Chandra}},\ }\bibfield  {title} {\bibinfo {title} {Studies of the magnetic
  structure of {FeSn} using the {M}\"ossbauer effect},\ }\href
  {https://doi.org/10.1088/0031-8949/11/1/008} {\bibfield  {journal} {\bibinfo
  {journal} {Physica Scripta}\ }\textbf {\bibinfo {volume} {11}},\ \bibinfo
  {pages} {47} (\bibinfo {year} {1975})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {H\"aggstr\"om}\ \emph {et~al.}(1974)\citenamefont
  {H\"aggstr\"om}, \citenamefont {Ericsson}, \citenamefont {W\"appling},
  \citenamefont {Karlsson},\ and\ \citenamefont
  {Chandra}}]{Haggstrom1974_MossbauerFeGe_FeSn_CoSn}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {L.}~\bibnamefont
  {H\"aggstr\"om}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Ericsson}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {W\"appling}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Karlsson}},\ and\ \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Chandra}},\ }\bibfield  {title} {\bibinfo {title} {{M}\"ossbauer studies of
  the isostructural compounds {FeGe}, {FeSn} and {CoSn}},\ }\href
  {https://doi.org/10.1051/jphyscol:19746129} {\bibfield  {journal} {\bibinfo
  {journal} {Le Journal de Physique Colloques}\ }\textbf {\bibinfo {volume}
  {35}},\ \bibinfo {pages} {C6} (\bibinfo {year} {1974})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Lin}\ \emph {et~al.}(2019)\citenamefont {Lin},
  \citenamefont {Wang}, \citenamefont {Wang}, \citenamefont {Yi}, \citenamefont
  {Li}, \citenamefont {Zhang}, \citenamefont {Wang}, \citenamefont {Wang},
  \citenamefont {Sun}, \citenamefont {Sun}, \citenamefont {Cho}, \citenamefont
  {Zeng},\ and\ \citenamefont {Zhang}}]{Lin2019_DiracInFeSn}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Z.}~\bibnamefont
  {Lin}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Wang}}, \bibinfo
  {author} {\bibfnamefont {P.}~\bibnamefont {Wang}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {Yi}}, \bibinfo {author} {\bibfnamefont
  {L.}~\bibnamefont {Li}}, \bibinfo {author} {\bibfnamefont {Q.}~\bibnamefont
  {Zhang}}, \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Wang}},
  \bibinfo {author} {\bibfnamefont {Z.}~\bibnamefont {Wang}}, \bibinfo {author}
  {\bibfnamefont {Y.}~\bibnamefont {Sun}}, \bibinfo {author} {\bibfnamefont
  {Z.}~\bibnamefont {Sun}}, \bibinfo {author} {\bibfnamefont {J.-H.}\
  \bibnamefont {Cho}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont
  {Zeng}},\ and\ \bibinfo {author} {\bibfnamefont {Z.}~\bibnamefont {Zhang}},\
  }\bibfield  {title} {\bibinfo {title} {Dirac fermions in antiferromagnetic
  {F}e{S}n {K}agome lattices with combined space inversion and time reversal
  symmetry},\ }\href@noop {} {\  (\bibinfo {year} {2019})},\ \Eprint
  {https://arxiv.org/abs/1906.05755v1} {1906.05755v1} \BibitemShut {NoStop}%
\bibitem [{\citenamefont {Djega-Mariadassou}\ \emph {et~al.}(1969)\citenamefont
  {Djega-Mariadassou}, \citenamefont {Lecocq},\ and\ \citenamefont
  {Michel}}]{DjegaMariadassou1969_MSn2+MSn}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.}~\bibnamefont
  {Djega-Mariadassou}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Lecocq}},\ and\ \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Michel}},\ }\bibfield  {title} {\bibinfo {title} {\'{E}tude magn\'etique et
  structurale des phases ${M}${S}n$_2$ et ${M}${S}n (${M}$ = {F}e, {C}o) et des
  solutions solides ({F}e$_x$${M}_{1-x}$){S}n, ({F}e$_x$${M}_{1-x}$){S}n$_2$
  (${M}$={C}o, {N}i)},\ }\href@noop {} {\bibfield  {journal} {\bibinfo
  {journal} {Annales de Chimie}\ }\textbf {\bibinfo {volume} {4}},\ \bibinfo
  {pages} {175} (\bibinfo {year} {1969})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Okamoto}(1999)}]{Ni-In_ASM1600357}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {H.}~\bibnamefont
  {Okamoto}},\ }\bibinfo {title} {{I}n-{N}i ({I}ndium-{N}ickel)}\ (\bibinfo
  {publisher} {Springer Science \& Business Media},\ \bibinfo {year} {1999})\
  p.\ \bibinfo {pages} {540}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Richter}(1998)}]{Richter1998_In-Ni-Sb}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {K.~W.}\ \bibnamefont
  {Richter}},\ }\bibfield  {title} {\bibinfo {title} {The ternary
  {I}n-{N}i-{S}b phase diagram in the vicinity of the binary {I}n-{N}i
  system},\ }\href {https://doi.org/10.1361/105497198770341941} {\bibfield
  {journal} {\bibinfo  {journal} {Journal of Phase Equilibria}\ }\textbf
  {\bibinfo {volume} {19}},\ \bibinfo {pages} {455} (\bibinfo {year}
  {1998})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hammond}(2005)}]{lide2005_CRCHandbook_ChTheElements}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.~R.}\ \bibnamefont
  {Hammond}},\ }\bibinfo {title} {{CRC} handbook of chemistry and physics}\
  (\bibinfo  {publisher} {CRC Press},\ \bibinfo {address} {Boca Raton},\
  \bibinfo {year} {2005})\ Chap.\ \bibinfo {chapter} {The elements},\ \bibinfo
  {edition} {eighty sixth}\ ed.\BibitemShut {Stop}%
\bibitem [{\citenamefont {Canfield}\ \emph {et~al.}(2016)\citenamefont
  {Canfield}, \citenamefont {Kong}, \citenamefont {Kaluarachchi},\ and\
  \citenamefont {Jo}}]{Canfield2016_CanfieldCrucibleSet}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {P.~C.}\ \bibnamefont
  {Canfield}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Kong}},
  \bibinfo {author} {\bibfnamefont {U.~S.}\ \bibnamefont {Kaluarachchi}},\ and\
  \bibinfo {author} {\bibfnamefont {N.~H.}\ \bibnamefont {Jo}},\ }\bibfield
  {title} {\bibinfo {title} {Use of frit-disc crucibles for routine and
  exploratory solution growth of single crystalline samples},\ }\href
  {https://doi.org/10.1080/14786435.2015.1122248} {\bibfield  {journal}
  {\bibinfo  {journal} {Philosophical Magazine}\ }\textbf {\bibinfo {volume}
  {96}},\ \bibinfo {pages} {84} (\bibinfo {year} {2016})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Okamoto}(1990{\natexlab{a}})}]{Pb-Rh_ASM901860}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {H.}~\bibnamefont
  {Okamoto}},\ }\bibinfo {title} {{B}inary alloy phase diagrams}\ (\bibinfo
  {year} {1990})\ Chap.\ \bibinfo {chapter} {{P}b-{R}h ({L}ead-{R}hodium)}, p.\
  \bibinfo {pages} {3005},\ \bibinfo {edition} {ii}\ ed.\BibitemShut {Stop}%
\bibitem [{\citenamefont {Okamoto}(1990{\natexlab{b}})}]{Pt-Tl_ASM901955}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {H.}~\bibnamefont
  {Okamoto}},\ }\bibinfo {title} {{B}inary alloy phase diagrams}\ (\bibinfo
  {year} {1990})\ Chap.\ \bibinfo {chapter} {{P}t-{T}l
  ({P}latinum-{T}hallium)}, p.\ \bibinfo {pages} {314305},\ \bibinfo {edition}
  {ii}\ ed.\BibitemShut {Stop}%
\bibitem [{\citenamefont {Bhan}\ \emph {et~al.}(1968)\citenamefont {Bhan},
  \citenamefont {G\"odecke}, \citenamefont {Panday},\ and\ \citenamefont
  {Schubert}}]{Bhan1968_Pd-Tl_Pt-Tl}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Bhan}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {G\"odecke}},
  \bibinfo {author} {\bibfnamefont {P.~K.}\ \bibnamefont {Panday}},\ and\
  \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Schubert}},\ }\bibfield
  {title} {\bibinfo {title} {Über die mischungen palladium-thallium und
  platin-thallium},\ }\href {https://doi.org/10.1016/0022-5088(68)90140-9}
  {\bibfield  {journal} {\bibinfo  {journal} {Journal of the Less Common
  Metals}\ }\textbf {\bibinfo {volume} {16}},\ \bibinfo {pages} {415} (\bibinfo
  {year} {1968})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Perdew}\ \emph {et~al.}(1996)\citenamefont {Perdew},
  \citenamefont {Burke},\ and\ \citenamefont {Ernzerhof}}]{Perdew1996_GGA}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~P.}\ \bibnamefont
  {Perdew}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Burke}},\ and\
  \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Ernzerhof}},\ }\bibfield
  {title} {\bibinfo {title} {Generalized gradient approximation made simple},\
  }\href {https://doi.org/10.1103/physrevlett.77.3865} {\bibfield  {journal}
  {\bibinfo  {journal} {Physical Review Letters}\ }\textbf {\bibinfo {volume}
  {77}},\ \bibinfo {pages} {3865} (\bibinfo {year} {1996})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Kresse}\ and\ \citenamefont
  {Furthm\"uller}(1996)}]{Kresse1996_AbInitioEnergyCalculations}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Kresse}}\ and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Furthm\"uller}},\ }\bibfield  {title} {\bibinfo {title} {Efficiency of
  ab-initio total energy calculations for metals and semiconductors using a
  plane-wave basis set},\ }\href {https://doi.org/10.1016/0927-0256(96)00008-0}
  {\bibfield  {journal} {\bibinfo  {journal} {Computational Materials Science}\
  }\textbf {\bibinfo {volume} {6}},\ \bibinfo {pages} {15} (\bibinfo {year}
  {1996})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kresse}\ and\ \citenamefont
  {Joubert}(1999)}]{Kresse1999_ProjectorAugmentedWaveMethod}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Kresse}}\ and\ \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Joubert}},\ }\bibfield  {title} {\bibinfo {title} {From ultrasoft
  pseudopotentials to the projector augmented-wave method},\ }\href
  {https://doi.org/10.1103/physrevb.59.1758} {\bibfield  {journal} {\bibinfo
  {journal} {Physical Review B}\ }\textbf {\bibinfo {volume} {59}},\ \bibinfo
  {pages} {1758} (\bibinfo {year} {1999})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Steinemann}\ \emph {et~al.}(1997)\citenamefont
  {Steinemann}, \citenamefont {Anongba},\ and\ \citenamefont
  {Podloucky}}]{Steinemann1997_ColorInPettiforsStructureMaps}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.~G.}\ \bibnamefont
  {Steinemann}}, \bibinfo {author} {\bibfnamefont {P.~N.~B.}\ \bibnamefont
  {Anongba}},\ and\ \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {Podloucky}},\ }\bibfield  {title} {\bibinfo {title} {Color in {P}ettifor's
  structure maps: intermetallic compounds for a new use},\ }\href
  {https://doi.org/10.1007/bf02665825} {\bibfield  {journal} {\bibinfo
  {journal} {Journal of Phase Equilibria}\ }\textbf {\bibinfo {volume} {18}},\
  \bibinfo {pages} {655} (\bibinfo {year} {1997})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Steinemann}\ \emph {et~al.}(2002)\citenamefont
  {Steinemann}, \citenamefont {Wolf},\ and\ \citenamefont
  {Podloucky}}]{Steinemann2002_IntermetallicsColorAndOpticalProperties}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.~G.}\ \bibnamefont
  {Steinemann}}, \bibinfo {author} {\bibfnamefont {W.}~\bibnamefont {Wolf}},\
  and\ \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Podloucky}},\
  }\bibfield  {title} {\bibinfo {title} {Color and optical properties},\
  }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Intermetallic
  Compounds--Principles and Practice}\ }\textbf {\bibinfo {volume} {3}},\
  \bibinfo {pages} {231} (\bibinfo {year} {2002})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Larsson}\ \emph {et~al.}(1974)\citenamefont
  {Larsson}, \citenamefont {Bystr\"om}, \citenamefont {Marklund},\ and\
  \citenamefont {Lindqvist}}]{Larsson1974_SpecificHeat_FeGe_FeSn_CoSn}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Larsson}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Bystr\"om}},
  \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Marklund}},\ and\
  \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Lindqvist}},\ }\bibfield
  {title} {\bibinfo {title} {Specific heat measurements of the {FeGe}, {FeSn}
  and {CoSn} compounds between 0.5 and 9 {K}},\ }\href
  {https://doi.org/10.1088/0031-8949/9/1/008} {\bibfield  {journal} {\bibinfo
  {journal} {Physica Scripta}\ }\textbf {\bibinfo {volume} {9}},\ \bibinfo
  {pages} {51} (\bibinfo {year} {1974})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kakihana}\ \emph {et~al.}(2019)\citenamefont
  {Kakihana}, \citenamefont {Nishimura}, \citenamefont {Aoki}, \citenamefont
  {Nakamura}, \citenamefont {Nakashima}, \citenamefont {Amako}, \citenamefont
  {Takeuchi}, \citenamefont {Kida}, \citenamefont {Tahara}, \citenamefont
  {Hagiwara}, \citenamefont {Harima}, \citenamefont {Hedo}, \citenamefont
  {Nakama},\ and\ \citenamefont
  {\=Onuki}}]{Kakihana2019_ElectronicStatesFeSn+CoSn}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Kakihana}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Nishimura}},
  \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Aoki}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Nakamura}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Nakashima}}, \bibinfo {author}
  {\bibfnamefont {Y.}~\bibnamefont {Amako}}, \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {Takeuchi}}, \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {Kida}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Tahara}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Hagiwara}},
  \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Harima}}, \bibinfo
  {author} {\bibfnamefont {M.}~\bibnamefont {Hedo}}, \bibinfo {author}
  {\bibfnamefont {T.}~\bibnamefont {Nakama}},\ and\ \bibinfo {author}
  {\bibfnamefont {Y.}~\bibnamefont {\=Onuki}},\ }\bibfield  {title} {\bibinfo
  {title} {Electronic states of antiferromagnet {FeSn} and {P}auli paramagnet
  {CoSn}},\ }\href {https://doi.org/10.7566/jpsj.88.014705} {\bibfield
  {journal} {\bibinfo  {journal} {Journal of the Physical Society of Japan}\
  }\textbf {\bibinfo {volume} {88}},\ \bibinfo {pages} {014705} (\bibinfo
  {year} {2019})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Marder}(2010)}]{Marder_CondensedMatterPhysics}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.~P.}\ \bibnamefont
  {Marder}},\ }\href@noop {} {\emph {\bibinfo {title} {Condensed matter
  physics}}},\ \bibinfo {edition} {2nd}\ ed.\ (\bibinfo  {publisher} {John
  Wiley and Sons, Hoboken, NJ},\ \bibinfo {year} {2010})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Mu}\ \emph {et~al.}(2019)\citenamefont {Mu},
  \citenamefont {Samolyuk}, \citenamefont {Wimmer}, \citenamefont
  {Troparevsky}, \citenamefont {Khan}, \citenamefont {Mankovsky}, \citenamefont
  {Ebert},\ and\ \citenamefont
  {Stocks}}]{Mu2019_ElectronScatteringMechanismsInNiFeCoCrMnHighEntropyAlloy}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Mu}}, \bibinfo {author} {\bibfnamefont {G.~D.}\ \bibnamefont {Samolyuk}},
  \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Wimmer}}, \bibinfo
  {author} {\bibfnamefont {M.~C.}\ \bibnamefont {Troparevsky}}, \bibinfo
  {author} {\bibfnamefont {S.~N.}\ \bibnamefont {Khan}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {Mankovsky}}, \bibinfo {author}
  {\bibfnamefont {H.}~\bibnamefont {Ebert}},\ and\ \bibinfo {author}
  {\bibfnamefont {G.~M.}\ \bibnamefont {Stocks}},\ }\bibfield  {title}
  {\bibinfo {title} {Uncovering electron scattering mechanisms in {NiFeCoCrMn}
  derived concentrated solid solution and high entropy alloys},\ }\bibfield
  {journal} {\bibinfo  {journal} {npj Computational Materials}\ }\textbf
  {\bibinfo {volume} {5}},\ \href {https://doi.org/10.1038/s41524-018-0138-z}
  {10.1038/s41524-018-0138-z} (\bibinfo {year} {2019})\BibitemShut {NoStop}%
\bibitem [{\citenamefont
  {Butler}(1985)}]{Butler1985_TheoryOfElectronicTransportInRandomAlloys}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {W.~H.}\ \bibnamefont
  {Butler}},\ }\bibfield  {title} {\bibinfo {title} {Theory of electronic
  transport in random alloys: {K}orringa-{K}ohn-{R}ostoker coherent-potential
  approximation},\ }\href {https://doi.org/10.1103/physrevb.31.3260} {\bibfield
   {journal} {\bibinfo  {journal} {Physical Review B}\ }\textbf {\bibinfo
  {volume} {31}},\ \bibinfo {pages} {3260} (\bibinfo {year}
  {1985})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Samolyuk}\ \emph {et~al.}(2019)\citenamefont
  {Samolyuk}, \citenamefont {Homes}, \citenamefont {May}, \citenamefont {Mu},
  \citenamefont {Jin}, \citenamefont {Bei}, \citenamefont {Stocks},\ and\
  \citenamefont
  {Sales}}]{Samolyuk2019_OpticalConductivityOfMetalAlloysWithResisdualResistivitiesNearMIRLimit}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.~D.}\ \bibnamefont
  {Samolyuk}}, \bibinfo {author} {\bibfnamefont {C.~C.}\ \bibnamefont {Homes}},
  \bibinfo {author} {\bibfnamefont {A.~F.}\ \bibnamefont {May}}, \bibinfo
  {author} {\bibfnamefont {S.}~\bibnamefont {Mu}}, \bibinfo {author}
  {\bibfnamefont {K.}~\bibnamefont {Jin}}, \bibinfo {author} {\bibfnamefont
  {H.}~\bibnamefont {Bei}}, \bibinfo {author} {\bibfnamefont {G.~M.}\
  \bibnamefont {Stocks}},\ and\ \bibinfo {author} {\bibfnamefont {B.~C.}\
  \bibnamefont {Sales}},\ }\bibfield  {title} {\bibinfo {title} {Optical
  conductivity of metal alloys with residual resistivities near or above the
  {M}ott-{I}offe-{R}egel limit},\ }\bibfield  {journal} {\bibinfo  {journal}
  {Physical Review B}\ }\textbf {\bibinfo {volume} {100}},\ \href
  {https://doi.org/10.1103/physrevb.100.075128} {10.1103/physrevb.100.075128}
  (\bibinfo {year} {2019})\BibitemShut {NoStop}%
\bibitem [{\citenamefont
  {Nikolaev}(2018)}]{Nikolaev2018_LandauDiamagMetalFermiSurface}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.~V.}\ \bibnamefont
  {Nikolaev}},\ }\bibfield  {title} {\bibinfo {title} {Landau diamagnetic
  response in metals as a {F}ermi surface effect},\ }\bibfield  {journal}
  {\bibinfo  {journal} {Physical Review B}\ }\textbf {\bibinfo {volume} {98}},\
  \href {https://doi.org/10.1103/physrevb.98.224417}
  {10.1103/physrevb.98.224417} (\bibinfo {year} {2018})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Jaccarino}\ \emph {et~al.}(1967)\citenamefont
  {Jaccarino}, \citenamefont {Wertheim}, \citenamefont {Wernick}, \citenamefont
  {Walker},\ and\ \citenamefont {Arajs}}]{Jaccarino1967_ParamagnetismFeSi}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {V.}~\bibnamefont
  {Jaccarino}}, \bibinfo {author} {\bibfnamefont {G.~K.}\ \bibnamefont
  {Wertheim}}, \bibinfo {author} {\bibfnamefont {J.~H.}\ \bibnamefont
  {Wernick}}, \bibinfo {author} {\bibfnamefont {L.~R.}\ \bibnamefont
  {Walker}},\ and\ \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Arajs}},\ }\bibfield  {title} {\bibinfo {title} {Paramagnetic excited state
  of {FeSi}},\ }\href {https://doi.org/10.1103/physrev.160.476} {\bibfield
  {journal} {\bibinfo  {journal} {Physical Review}\ }\textbf {\bibinfo {volume}
  {160}},\ \bibinfo {pages} {476} (\bibinfo {year} {1967})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Sales}\ \emph {et~al.}(1994)\citenamefont {Sales},
  \citenamefont {Jones}, \citenamefont {Chakoumakos}, \citenamefont
  {Fernandez-Baca}, \citenamefont {Harmon}, \citenamefont {Sharp},\ and\
  \citenamefont {Volckmann}}]{Sales1994_MagneticTrasportStruct_FeIrSi}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.~C.}\ \bibnamefont
  {Sales}}, \bibinfo {author} {\bibfnamefont {E.~C.}\ \bibnamefont {Jones}},
  \bibinfo {author} {\bibfnamefont {B.~C.}\ \bibnamefont {Chakoumakos}},
  \bibinfo {author} {\bibfnamefont {J.~A.}\ \bibnamefont {Fernandez-Baca}},
  \bibinfo {author} {\bibfnamefont {H.~E.}\ \bibnamefont {Harmon}}, \bibinfo
  {author} {\bibfnamefont {J.~W.}\ \bibnamefont {Sharp}},\ and\ \bibinfo
  {author} {\bibfnamefont {E.~H.}\ \bibnamefont {Volckmann}},\ }\bibfield
  {title} {\bibinfo {title} {Magnetic, transport, and structural properties of
  {Fe}$_{1-x}${Ir}$_x${Si}},\ }\href {https://doi.org/10.1103/physrevb.50.8207}
  {\bibfield  {journal} {\bibinfo  {journal} {Physical Review B}\ }\textbf
  {\bibinfo {volume} {50}},\ \bibinfo {pages} {8207} (\bibinfo {year}
  {1994})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Mandrus}\ \emph {et~al.}(1995)\citenamefont
  {Mandrus}, \citenamefont {Sarrao}, \citenamefont {Migliori}, \citenamefont
  {Thompson},\ and\ \citenamefont {Fisk}}]{Mandrus1995_ThermodynamicsOfFeSi}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Mandrus}}, \bibinfo {author} {\bibfnamefont {J.~L.}\ \bibnamefont {Sarrao}},
  \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Migliori}}, \bibinfo
  {author} {\bibfnamefont {J.~D.}\ \bibnamefont {Thompson}},\ and\ \bibinfo
  {author} {\bibfnamefont {Z.}~\bibnamefont {Fisk}},\ }\bibfield  {title}
  {\bibinfo {title} {Thermodynamics of {FeSi}},\ }\href
  {https://doi.org/10.1103/physrevb.51.4763} {\bibfield  {journal} {\bibinfo
  {journal} {Physical Review B}\ }\textbf {\bibinfo {volume} {51}},\ \bibinfo
  {pages} {4763} (\bibinfo {year} {1995})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Sales}\ \emph {et~al.}(2010)\citenamefont {Sales},
  \citenamefont {McGuire}, \citenamefont {Sefat},\ and\ \citenamefont
  {Mandrus}}]{Sales2010_SemimetalModelBaFeCo2As2}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.~C.}\ \bibnamefont
  {Sales}}, \bibinfo {author} {\bibfnamefont {M.~A.}\ \bibnamefont {McGuire}},
  \bibinfo {author} {\bibfnamefont {A.~S.}\ \bibnamefont {Sefat}},\ and\
  \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Mandrus}},\ }\bibfield
  {title} {\bibinfo {title} {A semimetal model of the normal state magnetic
  susceptibility and transport properties of
  {Ba}({Fe}$_{1-x}${Co}$_x$)$_2${As}$_2$},\ }\href
  {https://doi.org/10.1016/j.physc.2010.01.043} {\bibfield  {journal} {\bibinfo
   {journal} {Physica C: Superconductivity}\ }\textbf {\bibinfo {volume}
  {470}},\ \bibinfo {pages} {304} (\bibinfo {year} {2010})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Ashcroft}\ and\ \citenamefont
  {Mermin}(1976)}]{AshcroftMermin1976_SolidStatePhysics}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {N.~W.}\ \bibnamefont
  {Ashcroft}}\ and\ \bibinfo {author} {\bibfnamefont {N.~D.}\ \bibnamefont
  {Mermin}},\ }\href
  {https://www.ebook.de/de/product/3237015/neil_w_ashcroft_n_mermin_solid_state_physics.html}
  {\emph {\bibinfo {title} {Solid state physics}}}\ (\bibinfo  {publisher}
  {Brooks Cole Thomson Learning, London, UK},\ \bibinfo {year}
  {1976})\BibitemShut {NoStop}%
\end{thebibliography}%

